Evolution-aware VAriance (EVA) Coreset Selection for Medical Image Classification

In the medical field, managing high-dimensional massive medical imaging data and performing reliable medical analysis from it is a critical challenge, especially in resource-limited environments such as remote medical facilities and mobile devices. This necessitates effective dataset compression techniques to reduce storage, transmission, and computational cost. However, existing coreset selection methods are primarily designed for natural image datasets, and exhibit doubtful effectiveness when applied to medical image datasets due to challenges such as intra-class variation and inter-class similarity. In this paper, we propose a novel coreset selection strategy termed as Evolution-aware VAriance (EVA), which captures the evolutionary process of model training through a dual-window approach and reflects the fluctuation of sample importance more precisely through variance measurement. Extensive experiments on medical image datasets demonstrate the effectiveness of our strategy over previous SOTA methods, especially at high compression rates. EVA achieves 98.27% accuracy with only 10% training data, compared to 97.20% for the full training set. None of the compared baseline methods can exceed Random at 5% selection rate, while EVA outperforms Random by 5.61%, showcasing its potential for efficient medical image analysis.

==> paragraphs/tabs/tab_2.tex <==
\begin{table*}[!t]
    % \vspace{-5pt}
    \centering
    \caption{Different window combinations}
    % \caption{Per-split accuracies on COCO. Many, Medium, and Few are the three splits of the test set based on the training imbalancedness. Overall means the full test set. MT: the short for MaskTune. The complete experimental results (Mean $\pm$ Std) of all baselines can be found in \cref{appendix: Completed Results of tab:per split}.}
    
%    \vspace{-5pt}
 \label{tab:per split}
    \resizebox{\textwidth}{!}{
    \setlength{\tabcolsep}{1mm}{
% \begin{tabular}{c|cccccc>{\columncolor{blue!20}}c>{\columncolor{blue!20}}c>{\columncolor{blue!20}}ccc>{\columncolor[HTML]{EFEFEF}}c}


\begin{tabular}{c|ccccccccccc>{\columncolor[HTML]{EFEFEF}}c}
% \begin{tabular}{p{0.075\textwidth}<{\centering}|p{0.06\textwidth}<{\centering}p{0.06\textwidth}<{\centering}p{0.06\textwidth}<{\centering}p{0.06\textwidth}<{\centering}p{0.06\textwidth}<{\centering}p{0.06\textwidth}<{\centering}p{0.06\textwidth}<{\centering}p{0.06\textwidth}<{\centering}p{0.06\textwidth}<{\centering}p{0.06\textwidth}<{\centering}p{0.06\textwidth}<{\centering}>{\columncolor[HTML]{EFEFEF}}p{0.06\textwidth}<{\centering}}
\toprule[1.5pt]
% \rotatebox[origin=c]{60}{\footnotesize Methods}  & \rotatebox[origin=c]{60}{\footnotesize CE}    & \rotatebox[origin=c]{60}{\footnotesize PaCO}  & \rotatebox[origin=c]{60}{\footnotesize BCL}   & \rotatebox[origin=c]{60}{\footnotesize IFL}   & \rotatebox[origin=c]{60}{\footnotesize DB}    & \rotatebox[origin=c]{60}{\footnotesize TDE}   & \rotatebox[origin=c]{60}{\footnotesize ETF-DR} & \rotatebox[origin=c]{60}{\footnotesize LfF}   & \rotatebox[origin=c]{60}{\footnotesize Focal} & \rotatebox[origin=c]{60}{\footnotesize JTT}   & \rotatebox[origin=c]{60}{\footnotesize MaskTune} & \cellcolor[HTML]{EFEFEF}\rotatebox[origin=c]{60}{\footnotesize \textbf{\method}}  \\
\rotatebox[origin=c]{0}{\footnotesize Method}  & \rotatebox[origin=c]{0}{\footnotesize ERM}    & \rotatebox[origin=c]{0}{\footnotesize PaCO}  & \rotatebox[origin=c]{0}{\footnotesize BCL}   & \rotatebox[origin=c]{0}{\footnotesize IFL}   & \rotatebox[origin=c]{0}{\footnotesize DB}    & \rotatebox[origin=c]{0}{\footnotesize TDE}   & \rotatebox[origin=c]{0}{\footnotesize EIIL} & \rotatebox[origin=c]{0}{\footnotesize ARL}   & \rotatebox[origin=c]{0}{\footnotesize GRASP} & \rotatebox[origin=c]{0}{\footnotesize JTT}   & \rotatebox[origin=c]{0}{\footnotesize MT} & \rotatebox[origin=c]{0}{\footnotesize \textbf{\method}} \\
\midrule[0.6pt]
\midrule[0.6pt]
Many    &67.21\%  & 67.45\% & 66.89\%  & \textbf{67.71\%}   & 67.35\%  &66.32\%  & 66.87\%    & 67.32\%  &  67.13\%   & 66.93\%   &  64.48\%  & \textbf{67.71\%} \\
Medium  &52.22\%   & 53.33\%   &  53.21\%   & 52.17\%   & 52.11\%   & 53.23\%  & 52.79\%& 53.34\%& 53.26\%   & 51.24\%   &  50.11\%    & \textbf{53.50\%} \\
Few     &37.10\%   &  36.23\% & 37.67\%  &  36.82\%  & 37.47\% &37.02\% & 37.06\% &       37.18\% &  37.29\%  & 36.48\%   &  33.27\%    & \textbf{42.09\%} \\
Overall & 62.52\% & 62.59\% & 62.93\% & 62.57\% & 62.72\% & 62.64\% & 62.61\%  & 62.48\% & 62.73\% & 62.32\% & 60.23\%    & \textbf{64.56\%} \\
%STD &       &       &       &       &       &       &        &       &       &       &          &      \\ 
\bottomrule[1.5pt]
\end{tabular}}}
% \vspace{-20pt}
\end{table*}

==> paragraphs/tabs/tab_3.tex <==

\begin{table*}[t]
\centering
\caption{Accuracy comparison on OrganAMNIST, OrganSMNIST, CIFAR-10, and TissueMNIST, where both class imbalance and subpopulation imbalance co-exist (Mean $\pm$ Std). Bold indicates the superior results. Performance under more imbalance settings. Bold indicates superior results.  (Left) Performance on COCO, CIFAR-100, and tieredImageNet where both class imbalance and subpopulation imbalance co-exist (Mean $\pm$ Std). (Right) Performance on datasets for spurious correlations. The worst group accuracy (Worst Acc) and the average accuracy (Mean Acc) is reported. The second column means whether using the group annotation on the training or validation set.}
%\vspace{-5pt}
\label{tab:coupled imb}
\begin{minipage}[t]{0.513\textwidth}
    \resizebox{1.015\textwidth}{!}{
% \begin{tabular}{p{2.8cm}<{\centering}|p{2.8cm}<{\centering}|p{2.8cm}<{\centering}|p{2.8cm}<{\centering}}
\begin{tabular}{c|c|c|c}
\toprule[1.5pt]
\rowcolor[HTML]{D8D8D8} 
\multicolumn{4}{c}{Setting: both subpopulation and class imbalance (Mean $\pm$ Std)}\\
\midrule[0.6pt]
\midrule[0.6pt]
%\multirow{2}{*}{Methods} & \multicolumn{1}{c|}{\multirow{2}{*}{COCO}} & \multicolumn{3}{c|}{CIFAR-100}                    & \multirow{2}{*}{tieredImageNet} \\
%                        & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c}{IR = 100} & IR = 50 & IR = 20 &                              \\
Method & COCO & CIFAR-IR100 & tieredImageNet \\
\midrule[0.6pt]
\midrule[0.6pt]
ERM                      & 63.57 $\pm$ 0.34\%   & 59.24 $\pm$ 0.46\%& 53.65 $\pm$ 0.46\%     \\
LA						& 66.47 $\pm$ 0.27\%   & 59.73 $\pm$ 0.27\%& 54.12 $\pm$ 0.35\%   \\
LDAM    & 66.32 $\pm$ 0.33\%   & 59.66 $\pm$ 0.26\%& 54.01 $\pm$ 0.51\%      \\
CB		& 66.17 $\pm$ 0.21\%   & 59.45 $\pm$ 0.36\%& 53.78 $\pm$ 0.21\%      \\
PaCO                    & 66.78 $\pm$ 0.41\%   & 59.87 $\pm$ 0.51\%& 54.15 $\pm$ 0.39\%   \\
BCL                     & 66.92 $\pm$ 0.26\%   & 59.78 $\pm$ 0.37\%& 54.23 $\pm$ 0.27\%   \\
IFL                     & 65.34 $\pm$ 0.52\%   & 59.44 $\pm$ 0.41\%& 53.88 $\pm$ 0.43\%   \\
DB                      & 66.43 $\pm$ 0.15\%   & 59.81 $\pm$ 0.29\%& 54.14 $\pm$ 0.30\%   \\
TDE                     & 66.12 $\pm$ 0.44\%   & 59.63 $\pm$ 0.34\%& 53.91 $\pm$ 0.28\%   \\
ETF-DR                  & 65.92 $\pm$ 0.26\%   & 59.71 $\pm$ 0.18\%& 54.07 $\pm$ 0.31\%   \\

\rowcolor[HTML]{EFEFEF} 
\textbf{\method$_{\mathrm{w/ LA}}$}                   & \textbf{68.11 $\pm$ 0.27\% }  & \textbf{61.67 $\pm$ 0.31\%} & \textbf{55.73 $\pm$ 0.22\%}     \\
\bottomrule[1.5pt]
\end{tabular}}
\vspace{-15pt}
\end{minipage}
\hfill
\begin{minipage}[t]{0.481\textwidth}
% \hspace{-5pt}
\resizebox{\textwidth}{!}{
% \begin{tabular}{p{2.8cm}<{\centering}|p{2.8cm}<{\centering}|p{2.8cm}<{\centering}|p{2.8cm}<{\centering}}
\begin{tabular}{c|c|c|c}
\toprule[1.5pt]
\rowcolor[HTML]{D8D8D8} 
\multicolumn{4}{c}{Setting: spurious correlation (Worst Acc / Mean Acc)}\\
\midrule[0.6pt]\midrule[0.6pt]
\multirow{2}{*}{Method}& Group Info& \multirow{2}{*}{CelebA} & \multirow{2}{*}{Waterbirds}\\
&(Train / Val)& & \\
\midrule[0.6pt]
\midrule[0.6pt]
GDRO & Yes / Yes  & \textbf{88.3\%} / 91.8\% & \textbf{91.4\%} / 93.5\%\\
       \midrule[0.6pt]
       LfF & No / Yes  & 77.2\% / 85.1\%  & 82.1\% / 94.3\%\\
       SD & No / Yes  & \textbf{83.2\%} / 91.6\% & \textbf{87.3\%} / 90.3\%\\
       JTT & No / Yes  & 81.1\% / 88.0\% & 86.7\% / 93.3\%\\
       CIM & No / Yes  & 81.3\% / 89.2\%  & 77.2\% / 95.6\%\\
        \midrule[0.6pt]
       ERM & No / No  &47.2\% / 95.6\%  & 74.9\% / 98.1\%\\
       LfF & No / No  &24.4\% / 85.1\%  & 67.5\% / 87.5\%\\
       JTT & No / No  &40.6\% / 88.0\%  & 71.8\% / 92.3\%\\
       MaskTune & No / No  & \textbf{78.0\%} / 91.3\%    & 80.7\% / 92.1\%\\
       \rowcolor[HTML]{EFEFEF} 
       \textbf{\method$_{\mathrm{ w/ GDRO}}$} & No / No  & 77.9\% / 91.7\% & \textbf{81.9\%}/ 91.3\%\\
       \bottomrule[1.5pt]
\end{tabular}
}
\vspace{-25pt}
\end{minipage}
% \vspace{-12pt}
% \hfill
% \midrule[1.5pt]\midrule[1.5pt]
\end{table*}


